Model-based Estimation of AV-nodal Refractory Period and Conduction Delay Trends from ECG

Atrial fibrillation (AF) is the most common arrhythmia, associated with significant burdens to patients and the healthcare system. The atrioventricular (AV) node plays a vital role in regulating heart rate during AF, but is often insufficient in regards to maintaining a healthy heart rate. Thus, the AV node properties are modified using rate-control drugs. Hence, quantifying individual differences in diurnal and short-term variability of AV-nodal function could aid in personalized treatment selection. This study presents a novel methodology for estimating the refractory period (RP) and conduction delay (CD) trends and their uncertainty in the two pathways of the AV node during 24 hours using non-invasive data. This was achieved using a network model together with a problem-specific genetic algorithm and an approximate Bayesian computation algorithm. Diurnal and short-term variability in the estimated RP and CD was quantified by the difference between the daytime and nighttime estimates and by the Kolmogorov-Smirnov distance between adjacent 10-minute segments in the 24-hour trends. Holter ECGs from 51 patients with permanent AF during baseline were analyzed, and the predictive power of variations in RP and CD on the resulting heart rate reduction after treatment with four rate control drugs was investigated. Diurnal variability yielded no correlation to treatment outcome, and no prediction of drug outcome was possible using the machine learning tools. However, a correlation between the short-term variability for the RP and CD in the fast pathway and resulting heart rate reduction during treatment with metoprolol ($\rho=0.48, p<0.005$ in RP, $\rho=0.35, p<0.05$ in CD) were found. The proposed methodology enables non-invasive estimation of the AV node properties during 24 hours, which may have the potential to assist in treatment selection.

==> CopyFile.tex <==
\begin{itemize}
\item Item1
\item Item2 
\end{itemize}


\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}


\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}




==> NotUsedText.tex <==
This $\Delta P$ is used to vary the four hyper-parameters $P_{C}$, $P_{M}^{Ind}$, $P_{M}^{E}$, $\sigma_{M}$ relating to the population diversity in order to match the current situation for the data. The number of generations the GA runs before taking a step in the data ($N_{Gen}^{Current}$) also varies depending on $\Delta P$, so that the algorithm can better track large changes and at the same time be able to save computing power where changes are small. This $N_{Gen}^{Current}$ changes between 1 when $\Delta P < 800$; to 2 when $800 <\Delta P < 2000$; to 3 when $2000 < \Delta P$. The four hyper-parameters were set to change according to Equation \ref{Eq:Hyper},

\small
\begin{equation} \label{Eq:Hyper}
\begin{multlined}
    H_{Min} \ if\ \Delta P < 400, \\
    H_{Min} + \frac{H_{Mean} - H_{Min}}{1000 - 400}(\Delta P - 400) \ if\ 400 < \Delta P < 1000, \\
    H_{Mean} + \frac{H_{Max} - H_{Mean}}{5000 - 1000}(\Delta P - 1000) \ if\ 1000 < \Delta P < 5000, \\
H_{Max} \ if\ 5000 < \Delta P,
\end{multlined}
\end{equation}
\normalsize 

where the values for $H_{Min}$, $H_{Mean}$ and $H_{Max}$ for the different hyper-parameters can be seen in Table \ref{Tab:Hyper}.

\begin{table}[H]
\centering
\caption{Ranges for the hyper-parameters that changes depending on $\Delta P$.}
\begin{tabular}{ |c| m{1cm} m{1cm} m{1cm}|}
\hline
Parameter               & Minimum $H_{Min}$ & Mean $H_{Mean}$ & Maximum $H_{Max}$ \\ \hline
$P_{C}$             & 0.4 & 0.55 & 0.7 \\  
$P_{M}^{Ind}$  & 0.6 & 0.75 & 0.9 \\ 
$P_{M}^{E}$     & $\frac{1}{12}$ & $\frac{2}{12}$ & $\frac{5}{12}$ \\ 
$\sigma_{M}$           & 0.X & 0.X & 0.X \\ 
$N_{I}$        & 0.10 & 0.25 & 0.7 \\  \hline
\end{tabular}
\label{Tab:Hyper}
\end{table}


\begin{equation} \label{Eq:NLME}
\begin{multlined}
Y = M + A*cos( \frac{2\pi}{24}t + \phi  )



    Y_i = \theta_1 + d_V \theta_1^{V} + d_D \theta_1^{D} + d_M \theta_1^{M} + d_C \theta_1^{C} + \\
    \eta_1 + d_V \eta_1^{V} + d_D \eta_1^{D} + d_M \eta_1^{M} + d_C \eta_1^{C} + \\
    \big ( \theta_2 + d_V \theta_2^{V} + d_D \theta_2^{D} + d_M \theta_2^{M} + d_C \theta_2^{C} + \\
    \eta_2 + d_V \eta_2^{V} + d_D \eta_2^{D} + d_M \eta_2^{M} + d_C \eta_2^{C}  \big )cos( \frac{2\pi}{24}t + Phase ).
    \end{multlined}
\end{equation}


The effect of having a problem-specific GA with hyper-parameter tuning during the optimization, as well as using a complex immigration strategy are evaluated by comparing it with a more basic version of the GA. The hyper-parameters for this basic version were set to the $H_{Min}$ as seen in Table \ref{Tab:Hyper}. Moreover, $N_{Gen}^{Current}$ was also fixed to 2. To account for the slight difference in the total generation this leads to, the number of individuals in the population was slightly changed to assure that the two algorithms had the same running time. Five different patients, all with varying RR interval series characteristics, were used for this comparison. Each patient data were optimized with the respective GA ten times, and the average is shown in Table \ref{Tab:GAvsGA}.

The $\epsilon$ value for all patients, all drugs, and all window placements are jointly presented in Figure \ref{fig:PP_all}. Du to the difficulty in interpreting these numbers, we also include the Poincaré plots \textcolor{red}{and histograms?} of the model output and the data for the 50\% and 95\% case, which are shown in Figure \ref{fig:PP_2}.

The model output for even the 95\% worst estimated parameters closely resembles that of the data, however, as seen in \ref{fig:PP_all}, there are still a few instances where the model failed.


\begin{figure}[H]
    \centering
        \includegraphics[width=8cm]{Figures/Phase_OK.jpg}
    \caption{Phase for the circadian variance derived from the PCA analysis, with patient number on the x-axis and phase on the y-axis.}
    \label{fig:Res:Phase}
\end{figure}







In order to re-use previously individuals, the model output for the ten fittest individuals from each generation is saved, along with the current $\lambda$ value and $RR_{min}$. Then, for every new OS, the ten previous generations with the most similar $RR_{min}$ and $\lambda$, with respect to the current ones, are selected. From these, the saved individuals with the lowest $\epsilon$ evaluated using the current data are selected for immigration. The memory part of the immigration starts at generation ten, and is therefore replaced with method 3 - random samples - before that.

The individuals for method 2 are created from eight smaller GA, each with 16 individuals and a segment length $L$ of 750, that runs simultaneously as the main GA. The individuals with the highest fitness are then chosen to immigrate into the main GA. Note that this immigration does not remove individuals from the smaller GA, but copies them over to the main GA.

Method 3, random samples, are created in the same manner as for the population initialization, using a latin hypercube sampling in the range $\boldsymbol{r_p}$.
